Benchmarking Inverse Optimization Algorithms for Materials Design

Machine learning-based inverse materials discovery has attracted enormous attention recently due to its flexibility in dealing with black box models. Yet, many metaheuristic algorithms are not as widely applied to materials discovery applications as machine learning methods. There are ongoing challenges in applying different optimization algorithms to discover crystals with single- or multi-elemental compositions and how these algorithms differ in mining the ideal materials. We comprehensively compare 11 different optimization algorithms for the design of single- and multi-elemental crystals with targeted properties. By maximizing the bulk modulus and minimizing the Fermi energy through perturbing the parameterized elemental composition representations, we estimated the unique counts of elemental compositions, mean density scan of the objectives space, mean objectives and frequency distributed over the materials' representations and objectives. We found that nature-inspired algorithms contain more uncertainties in the defined elemental composition design tasks, which correspond to their dependency on multiple hyperparameters. Runge Kutta optimization (RUN) exhibits higher mean objectives whereas Bayesian optimization (BO) displayed low mean objectives compared with other methods. Combined with materials count and density scan, we propose that BO strives to approximate a more accurate surrogate of the design space by sampling more elemental compositions and hence have lower mean objectives, yet RUN will repeatedly sample the targeted elemental compositions with higher objective values. Our work shed light on the automated digital design of crystals with single- and multi-elemental compositions and is expected to elicit future studies on materials optimization such as composite and alloy design based on specific desired properties.

==> figurecap_backup.tex <==
figure 1: Schematic of the materials design process. {\bf(A)} The materials design process begins with specific applications, such as semiconductor devices. {\bf(B)} Based on the intended industrial usage, specific desired properties are identified, such as high bulk modulus and low Fermi energy. {\bf(C)} A digital design optimization problem is formulated using numerical models to discover or design materials with the desired properties. {\bf(D)} Different optimization methods use exploration/exploitation strategies to generate a design space for exploring the best materials. {\bf(E)} The ideal materials are extracted from the design space exploration and are ready for real-world applications. In this study, we mostly focus on {\bf C}, {\bf D}, and {\bf E}, where we formulate an optimization framework that enables the most current popular optimization methods to be applied for searching the desired molecular materials and compare different optimizations based on certain metrics. The eventually ``mined'' materials are then analyzed.
% ==========================================
figure 2: The schematic for the optimization benchmarking and different optimization algorithms employed in the study. {\bf(A)} The workflow for discovering molecular materials through the combination of graph neural network (as surrogate models to evaluate materials properties) and defined design variables randomization for selecting optimal materials with targeted properties. For details please see {\em Method}. {\bf(B)} The schematic for optimization through metaheuristic algorithms, begins with a set of random particles (or population) sampled in the design space, to iteratively update and eventually clustered around the globally optimal values, indicating searching for the good materials with desired properties. {\bf(C)} The schematic for materials discovery using deep reinforcement learning. The optimization is enabled through training a deep neural network as the ``agent'' to make optimal decisions, i.e., selecting the good materials. This selection process is enabled via the action as the output of the network. The action screens the materials database and finds the corresponding structure as input to the graph neural network as the environment. The environment then feeds back rewards (from the properties of the predicted material) back to the agent for making the best decisions. {\bf(D)} Bayesian optimization methods for molecular materials discovery. The method seeks to build up a surrogate model of the design space by employing Gaussian process regression and searching for the next material evaluations based on an acquisition function. One can extract good materials from the design space surrogate.
% =============================
figure 3: Design space exploration, objective values evaluation, and target design space count of benchmarking different optimizations for single molecular materials design. {\bf (A)} The overall design space benchmarking of all the 12 different optimizations employed, marked in different shapes and colors. The black dashed line indicates the boundary of our ``targeted design space'', where the black dot stands for the properties of silicon (Si). {\bf (B)} The objective value changes w.r.t. all the material evaluations. Since the objective value changes are visualized to contain strong fluctuations, the reduced-order plot, samples the mean value of every 11 material evaluations are visualized on the top-left corner to capture the general trend of the objective changes. The ``good'' trends with desired increasing objective values are marked in bold lines. {\bf (C)} The number counts of the evaluated materials that land in the targeted design space of the 12 different optimization algorithms. The corresponding numbers are marked on top of the barplot. Note that the simplification: BO, GA, PSO, GWO, HIWOA, ACO, DE, SA, BOA, AOA, RUN, and DRL, stand for Bayesian Optimization, Genetic Algorithm, Particle Swarm Optimization, Grey Wolf Optimization, Hybrid-Improved Whale Optimization Algorithm, Ant Colony Optimization, Differential Evolution, Simulated Annealing, Bees Optimization, Arithmetic Optimization, Runge Kutta Optimization, and Deep Reinforcement Learning.
% ==================
figure 4: The design space evaluation process for selected optimization methods. Subfigures {\bf A} and {\bf C} are selected based on results in Figure \ref{fig3}\textbf{C}: they have more evaluated materials in the targeted design space compared with other algorithms. Subfigures {\bf B} and {\bf D} are selected based on results in Figure \ref{fig3}\textbf{B}: they possess more evident objective value-increasing trends compared with other algorithms. The materials corresponding to the data point that is observed to be the closest to the Pareto front are also visualized in the center of each figure. Note that the color gradients of the data points stand for the material evaluation process w.r.t. time, marked in the color bar on the right. The contour plots on the bottom visualize the normalized design variables, in the scale of [0,1] marked on the right color bar.
% =================================
figure 5: The results of the optimization benchmarking. {\bf (A)} The probability distribution of the selected materials in the targeted design area from all the different optimization methods. The upper subfigure indicates the elements and the bottom subfigure indicate the detailed elemental composition. {\bf (B)} The objective values ($K$ and $-E_{\rm Fermi}$) distribution along the material evaluation process, marked in the range bounded by the properties of silicon. Note that those materials whose bulk modulus is smaller than or whose Fermi energy is larger than silicon's corresponding value are in black and ``filtered'' out. {\bf (C)} The reconstructed design space, i.e., The $K$ and $E_{\rm Fermi}$ values w.r.t. to two design variables $\xi_n$ and $\eta$ as the overall mean value of the 12 different optimization algorithms.
% ======================================
figure 6: Design space exploration, objective values evaluation, and target design space count of benchmarking different optimizations for multi-molecular materials design. {\bf (A)} The overall design space benchmarking of all the 12 different optimizations employed, marked in different shapes and colors. The black dashed line indicates the boundary of our ``targeted design space'', where the black dot stands for the properties of silicon (Si). {\bf (B)} The objective value changes w.r.t. all the material evaluations. Since the objective value changes are visualized to contain strong fluctuations, the reduced-order plot, samples the mean value of every 11 material evaluations are visualized on the top-left corner to capture the general trend of the objective changes. The ``good'' trends with desired increasing objective values are marked in bold lines. {\bf (C)} The number counts of the evaluated materials that land in the targeted design space of the 12 different optimization algorithms. The corresponding numbers are marked on top of the barplot.
% ============
figure 7: The design space evaluation process for selected optimization methods. Subfigures {\bf A}, {\bf B}, {\bf C}, and {\bf D} are selected based on results in Figure \ref{fig3}\textbf{B}: they possess more evident objective value-increasing trends compared with other algorithms. Subfigures {\bf D}, {\bf E} and {\bf F} are selected based on results in Figure \ref{fig3}\textbf{C}: they have more evaluated materials in the targeted design space compared with other algorithms. The materials corresponding to the data point that is observed to be the closest to the Pareto front are also visualized in the center of each figure. Note that the color gradients of the data points stand for the material evaluation process w.r.t. time, marked in the color bar on the right. The contour plots on the bottom visualize the normalized design variables, in the scale of [0,1] marked on the right color bar.
% =================
The results of multi-molecular materials design optimization and the overall objective mean values for both the single and multi-molecular materials design optimization. {\bf(A)} The extracted molecular materials and their probability distribution from all the multi-molecular materials optimization. All the materials with a count of more than 1 are highlighted on top of the bar. {\bf(B)} The objective values ($K$ and $-E_{\rm Fermi}$) distribution along the material evaluation process, marked in the range bounded by the properties of silicon. Note that those materials whose bulk modulus is smaller than or whose Fermi energy is larger than silicon's corresponding value are in black and ``filtered'' out. {\bf(C)} The mean objective values of the different optimization methods employed for both the single and multi-molecular materials design optimization cases. The upper subfigure is the single molecular materials optimization case and the bottom subfigure is the multi-molecular materials optimization case.
